Recover the lost Phasor Measurement Unit Data Using Alternating Direction Multipliers Method

This paper presents a novel algorithm for recovering missing data of phasor measurement units (PMUs). Due to the low-rank property of PMU data, missing measurement recovery can be formulated as a low-rank matrix-completion problem. Based on maximum-margin matrix factorization, we propose an efficient algorithm based on alternating direction method of multipliers (ADMM) for solving the matrix completion problem. Comparing to existing approaches, the proposed ADMM based algorithm does not need to estimate the rank of the target data matrix and provides better performance in computation complexity. In addition, we consider the case of measurements missing from all PMU channels and provide a strategy of reshaping the matrix which contains the received PMU data for recovery. Numerical results using PMU measurements from IEEE 68-bus power system model illustrate the effectiveness and efficiency of the proposed approaches.

==> bib_backup.tex <==

\bibitem{Phadke2008}
A. G. Phadke and J. S. Thorp, ``Synchronized Phasor Measurements and Their Applications," New York, Springer, 2008.

\bibitem{Chen2013}
Y. Chen, L. Xie, and P. Kumar, ``Dimensionality Reduction and Early Event Detection Using Online Synchrophasor Data," in {\it Proc. IEEE Power and Energy Society General Meeting}, pp. 1-5, 2013.

\bibitem{Dahal2012}
N. Dahal, R. L. King, and V. Madani, ``Online Dimension Reducion of Synchrophasor Data," in {\it Proc. IEEE PES Transmission and Distribution Conf. Expo. (T\& D)}, pp. 1-7, 2012.

\bibitem{Gao2014}
P. Gao, M. Wang, S. Ghiocel, and J. H. Chow, ``Modeless Reconstruction of Missing Synchrophasor Measurements," in {\it Proc. IEEE PES General Meeting}, 2014.


\bibitem{Candès2010}
E. J. Candes and T. Tao, ``The Power of Convex Relaxation: Near-Optimal Matrix Completion," {\it IEEE Transactions on Information Theory}, vol. 56, no. 5, pp. 2053-2080, 2010.

\bibitem{Mazumder2010}
R. Mazumder, H. Trevor, and T. Robert, ``Spectral Regularization Algorithms for Learning Large Incomplete Matrices," {\it Journal of machine learning research}, vol. 11, pp. 2287-2322, 2010.

\bibitem{Rennie2005}
J. D. Rennie and S. Nathan, ``Fast Maximum Margin Matrix Factorization for Collaborative Prediction." {\it in Proc. the 22nd international conference on Machine learning (ACM)}, 2005.

\bibitem{Chen2012}
C. Chen, B. He, and X. Yuan, ``Matrix Completion via an Alternating Direction Method," {\it IMA Journal of Numerical Analysis}, vol. 32, no. 1, pp. 227-245, 2012.

\bibitem{Xu2016}
F. Xu, and P. Pan, ``A New Algorithm for Positive Semidefinite Matrix Completion," {\it Journal of Applied Mathematics}, vol. 3, pp. 1-5, 2016.


\bibitem{Jain2013}
P. Jain, N. Praneeth, and S. Sujay, ``Low-Rank Matrix Completion Using Alternating Minimization." {\it in Proc. the forty-fifth annual ACM symposium on Theory of computing (ACM)}, 2013.


\bibitem{Hardt2014}
M. Hardt, ``Understanding Alternating Minimization for Matrix Completion," {\it Foundations of Computer Science (FOCS), 2014 IEEE 55th Annual Symposium}, 2014.

\bibitem{Hastie2015}
T. Hastie, R. Mazumder, J. D. Lee, and R. Zadeh, ``Matrix Completion and Low-Rank SVD via Fast Alternating Least Squares," {\it J. Mach. Learn. Res}, vol. 16, no. 1, pp. 3367-3402, 2015.

\bibitem{Gao2016}
P. Gao, M. Wang, S. G. Ghiocel, J. H. Chow, B. Fardanesh, and G. Stefopoulos, ``Missing Data Recovery by Exploiting Low-Dimensionality in Power System Synchrophasor Measurements," {\it IEEE Trans. on Power Systems}, vol. 31, no. 2, pp. 1006-1013, 2016.


\bibitem{Ouyang2013}
H. Ouyang, N. He, Q. T.  Long, and A. Gray, ``Stochastic Alternating Direction Method of Multipliers," {\it in Proc. International Conference on International Conference on Machine Learning}, pp. I-80, 2013.


\bibitem{Zhang2004}
X. Zhang, ``Matrix Analysis and Applications," {Tsinghua and Springer Publishing house}, Beijing, pp. 71-100, 2004.


\bibitem{PhD}
M. Fazel, ``Matrix Rank Minimization with Applications," Ph. D. dissertation, Stanford Univ., Stanford, CA, 2002. 
